Complexity of Model Checking Recursion Schemes for Fragments of the Modal Mu-Calculus

Ong has shown that the modal mu-calculus model checking problem (equivalently, the alternating parity tree automaton (APT) acceptance problem) of possibly-infinite ranked trees generated by order-n recursion schemes is n-EXPTIME complete. We consider two subclasses of APT and investigate the complexity of the respective acceptance problems. The main results are that, for APT with a single priority, the problem is still n-EXPTIME complete; whereas, for APT with a disjunctive transition function, the problem is (n-1)-EXPTIME complete. This study was motivated by Kobayashi's recent work showing that the resource usage verification of functional programs can be reduced to the model checking of recursion schemes. As an application, we show that the resource usage verification problem is (n-1)-EXPTIME complete.

==> equivalence.tex <==
% !TEX root = Main.tex
%\documentclass[a4paper]{lmcs}
%\usepackage{paralist,amssymb,url,bcprules}
%\usepackage[usenames]{color}
%\input{local}
%\newcommand\todo[1]{{\footnotesize \color{OliveGreen}
%[\textbf{To do:} #1]}}
%\newcommand\nk[1]{{\footnotesize \color{blue}
%[#1 - \textbf{Naoki}]}}
%\newcommand\lo[1]{\marginpar[{\color{red}\small\dbend}]{
%\color{red}\small\dbend}{\footnotesize \color{red}
%[#1 - \textbf{Luke}]}}
%\newcommand\changed[1]{{\color{blue}{#1}}}
%\newcommand\lochanged[1]{{\color{red}{#1}}}
%
%\begin{document}
\section{On the Equivalence between the Two Definitions of APT} \label{apx:equivalence}
\newcommand\APTe{APT\(_{\epsilon}\)}
We call  \APTe{} for the APT as defined in Appendix~\ref{apx:APT_mucalculus}
and just call APT for the APT in Section 2.
%The acceptance condition for \APTe{} is not explicitly stated in Appendix, but it should be essentially the same: we can define a run tree analogously, and a run tree is accepting just if, for every infinite path of the run tree, the largest priorities that occur infinitely often is even. 
\nk{I am not sure how you intended to define acceptance conditions to take \(\top\) and \(\bot\) into account: Do we require that the priority of \(\top\) is even and that of \(\bot\) is odd? But then, trivial \APTe{} cannot have a \(\bot\) state. Why did you introduce \(\top\) and \(\bot\) and require that the image of \(\delta\) is non-empty, instead of requiring that \(\top\) and \(\bot\) are respectively existential and universal states and \(\delta(\top,f) =\delta(\bot,f) = \emptyset\)?}
\lo{Thanks for your questions and comments. The revised definition does not require distinguished states $\top$ and $\bot$.}
The translation from APT to \APTe{} is obvious.
Let \((\Sigma, Q, \delta, q_I, \Omega)\) be an APT.
For each \(\theta\) that occurs as a subformula of the codomain of \(\delta\),
introduce a new state \(q_\theta\), and define the transition \(\delta'\) by:
\[
\begin{array}{ll}
\delta'(q_j, f) = \set{(\epsilon, q_{\delta(q_j,f)})} & \mbox{if \(q_j\in Q\)}\\
\delta'(q_{\theta_1\land\theta_2},f) = \delta'(q_{\theta_1\lor\theta_2}) = \set{(\epsilon,q_{\theta_1}), (\epsilon,q_{\theta_2})}\\
\delta'(q_{(i,q_j)}, f) = \set{(i, q_j)}\\
\lochanged{\delta'(q_{\TRUE}, f) = \delta'(q_{\FALSE}, f) = \emptyset}\\
%\delta'(\top, f) = \set{(\epsilon,\top)}?\\
%\delta'(\bot, f) = \set{(\epsilon,\bot)}?\\
\end{array}
\]
\nk{I think it is simpler to remove the restriction that the image of \(\delta'\) is non-empty, and
set \(\delta'(q_{\TRUE}, f) = \delta'(q_{\FALSE}, f) = \emptyset\), if it does not affect the 
translations between modal mu-calculus.} \lo{I agree.}
Universal states are states of the form \(q_{\theta_1\land\theta_2}, \lochanged{q_{\TRUE}}\). \lo{At a move $(\alpha, q)$ of the acceptance game where $q$ is a universal state, \Abelard chooses the next move; since $\delta'(q_{\TRUE}, f) = \emptyset$, \Abelard is stuck, and so \Eloise wins.} All the other states are existential.

For the translation from \APTe{} to APT, we need to eliminate \(\epsilon\)-transitions.
Let \(\APT :=(\Sigma, Q, \delta, q_I, \Omega)\) be an \APTe{}.
We define the transition function \(\delta'\) of APT by using auxiliary transition functions
\(\delta^{(0)},\delta^{(1)},\ldots\) on states of the form \(q_{i_1}\cdots q_{i_k}\in Q^*\).
\[
\begin{array}{ll}
\delta^{(0)}(q_j, f) = \left\{
   \begin{array}{ll}
      \bigvee \delta(q_j,f) & \mbox{if $q_j$ is an existential state}\\
      \bigwedge \delta(q_j,f) & \mbox{if $q_j$ is a universal state}
   \end{array}\right.\\
\delta^{(i+1)}(q_j,f) = \rho\;\delta^{(i)} \\
\end{array}
\]
Here, \(\rho \; \delta^{(i)}\) is the formula obtained from \(\delta^{(i)}\) by replacing
each atomic formula of the form \((\epsilon,q_{\ell_1}\cdots q_{\ell_k})\) with:
\[
\begin{array}{l}
\rho(\epsilon, q_{\ell_1}\cdots q_{\ell_k}) :=
  \left\{ \begin{array}{ll}
      \bigvee \set{ (q_{\ell_1}\cdots q_{\ell_{k}})\odot \theta \mid \theta \in \delta(q_{\ell_k},f)}
%%\hat{\delta}(q_{\ell_1}\cdots q_{\ell_k},f) 
                 & \mbox{if $q_{\ell_k}$ is an existential state}\\
      \bigwedge \set{ (q_{\ell_1}\cdots q_{\ell_{k}})\odot \theta \mid \theta \in \delta(q_{\ell_k},f)}
                 & \mbox{if $q_{\ell_k}$ is a universal state}
   \end{array}\right.\\
q_{\ell_1}\cdots q_{\ell_k}\odot (j, q) = (j, q_{\ell_1}\cdots q_{\ell_k}q)\\
q_{\ell_1}\cdots q_{\ell_k}\odot (\epsilon, q) = 
  \left\{ \begin{array}{ll}
              (\epsilon, q_{\ell_1}\cdots q_{\ell_k}q) & \mbox{if $q\not\in \set{q_{\ell_1},\ldots, q_{\ell_k}}$}\\
              \TRUE & \mbox{if $q=q_{\ell_n}$ and the largest priority in \(q_{\ell_n}\cdots q_{k}\) is even}\\
              \FALSE & \mbox{if $q=q_{\ell_n}$ and the largest priority in \(q_{\ell_n}\cdots q_{k}\) is odd}\\
     \end{array}\right.
  \\
\end{array}
\]
Intuitively, we expand each \(\epsilon\)-transition until it is replaced by non-\(\epsilon\) transitions or
a cycle is found. In the latter case, we just replace the formula by \(\TRUE\) or \(\FALSE\), depending on
the largest priority in the cycle.

Define the transition function \(\delta'\) of APT by:
\[ \delta'(q_{\ell_1}\cdots q_{\ell_k},f) = \delta^{(|Q|)}(q_{\ell_k},f).\]
By the construction of \(\delta^{(i)}\) above,
\(\delta'\) does not contain an atomic formula of the form \((\epsilon,q_{\ell_1}\cdots q_{\ell_k})\). Thus,
\(\APT' := (\Sigma,Q^+,\delta',q_I,\Omega')\) is an APT, where \(\Omega'(q_{\ell_1}\cdots q_{\ell_k})\) is
the largest priority of \(q_{\ell_1},\ldots, q_{\ell_k})\).
Furthermore, if \(\APT\) is trivial (disjunctive, resp.), \(\APT'\) is also trivial (disjunctive, resp.).

It remains to check that \(\APT\) and \(\APT'\) are equivalent.
Suppose that \(T\) is accepted by \(\APT\). Then there exists an accepting run-tree \(R\) of \(\APT\).
Let \(R'\) be the tree obtained by ``shortcutting'' \(\epsilon\)-transitions
(for each node \((\pi, q)\), let its children be \((\pi j, q_{\ell_1}\cdots q_{\ell_k}q_j)\) such that there is a path from
  \((\pi, q)(\pi,q_{\ell_1}) \cdots (\pi,q_{\ell_k})(\pi j, q_j)\) in \(T\), and remove all the intermediate nodes).
Then, \(R'\) is an accepting run tree of \(\APT'\), hence \(T\) is accepted by \(\APT'\).

Conversely, suppose that \(T\) is accepted by \(\APT'\). 
Then there exists an accepting run-tree \(R'\) of \(\APT'\).
Let \(R\) be the tree obtained by ``expanding'' \(R'\)
(e.g., by expanding an edge \((\pi,q_{\ell_1}\cdots q_{\ell_k}) (\pi i, q_{\ell_k}q'_{\ell_1}\cdots q'_{\ell_{k'}})\)
to \((\pi,q_{\ell_k})(\pi,q'_{\ell_1})\cdots (\pi,q'_{\ell_{k'-1}})(\pi i, q'_{\ell_{k'}})\);
\changed{we also need paths representing infinite \(\epsilon\)-edges, so the details need to be worked out).}
Then \(R'\) is an accepting run-tree of \(\APT\), hence \(T\) is accepted by \(\APT\).

%\paragraph{\textbf{Remark}}
\begin{remark}
In the construction above, the number of states of \(\APT'\) can be exponential in the number of states
of \(\APT\). We can avoid it by replacing \(q_{\ell_1}\cdots q_{\ell_k}\) with \((q_{\ell_k}, m)\)
where \(m\) is the largest priority in \(q_{\ell_1}\cdots q_{\ell_k}\). It is not clear if we can easily avoid the exponential blow-up of the size of \(\delta'\).
\end{remark}
%\end{document}


==> path-9Feb.tex <==
\section{Disjunctive APT and Complexity of Model Checking}
\label{sec:disjunctiveAPT}

%%\nk{I have restructured this section to make the structure similar to
%%that of the previous section: first introduce a subclass of APT, and
%%then analyze the complexity of the model checking problem.} \lo{This
%%is fine.}

\newcommand\pathlang[1]{\mathcal{W}\,{#1}}
\newcommand\vp{\hbox{\bf VP}}
\newcommand\cgraph[1]{\mathit{Gr}_{#1}}

%%\section{(\(n-1\))-EXPTIME-Completeness of Verification of Path Properties}

\subsection{Disjunctive APT}

\lo{It seems a little odd that, in contrast to trivial APT, the logical characterization of disjunctive APT is relegated to Appendix~\ref{sec:equi-expressivity}. For this reason, and following the pattern of the preceding section, I have (i) inserted a subsection (ii) introduced the ``disjunctive fragment'' (iii) changed the footnote to a remark. If you are not happy with any of the above, please feel free to change it back.}

A \emph{disjunctive APT} is an APT whose transition function
\(\delta\) is disjunctive, i.e.~the image of \(\delta\) consists of positive boolean formulas that contain only disjunctions and no conjunctions, as given by the grammar
\(\theta \; ::= \; \TRUE \; | \; \FALSE \; | \; (i, q) \; | \;  \theta \vee \theta \).
Disjunctive APT can be used to describe path (or linear-time) properties of trees.

\lochanged{
First we give a logical characterization of disjunctive APT as follows. Call $\cal D$ the following ``disjunctive fragment'' of the modal mu-calculus:
\[\phi, \psi \; ::= \; P_f \wedge \phi
%\; | \; (\neg P_f) \wedge \phi
\; | \; Z
\; | \; \phi \vee \psi
\; | \; \diaform{i}{\phi}
\; | \; \nuform{Z}{\phi}
\; | \; \muform{Z}{\phi}
\]
where $f$ ranges over symbols in $\Sigma$, and $i$ ranges over $\set{1, \cdots, \arity(\Sigma)}$.
A proof is given in Appendix~\ref{sec:equi-expressivity}.
%}

\begin{proposition}[Equi-Expressivity]
\label{prop:equi-expressivity2}
The logic $\cal D$ and %%B\"uchi automata
disjunctive APT are equivalent for defining possibly-infinite
ranked trees. I.e.~for every closed $\cal D$-formula, there is a disjunctive APT that defines the same tree language, and vice versa.
\end{proposition}

\begin{remark}\rm \begin{inparaenum}[(i)]
\item Note that a disjunctive APT is a non-deterministic parity tree automaton.
\item For defining languages of ranked trees, disjunctive APT (or rather the formulas corresponding to them) are a proper subset of the \emph{disjunctive formulas} in the sense of Walukiewicz and Janin  \cite{JW95}. (Satisfiability checking of these disjunctive formulas is linear time.) For example, the disjunctive formula $(1 \rightarrow \set{{\sf t}}) \wedge (2 \rightarrow \set{{\sf t}})$ is not equivalent to any disjunctive APT.
\end{inparaenum}
\end{remark}
}
%\nk{I have moved the remark here, due to the lack of space.}
%%\lo{ICALP referees who are aware of Walukiewicz' notion of \emph{disjunctive formulas} would likely query its connexion with disjunctive APT, hence the remark. We could also insert it as a footnote.}
%%\end{remark}
%%%It follows from the definition of (disjunctive) APT that, in case
%%%$\arity(a) = 0$, it is possible for $\delta(q, a) \in {\sf
%%%B}^+(\emptyset)$ to be $\sf t$ or $\sf f$.}} \nk{Make it clear whether
%%%we allow \(\TRUE\) when the arity is \(0\).}\lo{Done.}
%%\nk{Actually, it seems that we can allow \(\TRUE\) even in the case \(\arity(a)\neq 0\). Am I right?} \lo{Yes.}
%%%We then use the result to analyze the complexity of
%%%decision problems on the \lochanged{\emph{path languages} (of trees)} generated by recursion schemes. See Appendix~\ref{sec:equi-expressivity} for a logical characterization of disjunctive APT.

In the rest of the section, we show that the model checking problem for order-\(n\) recursion schemes is \((n-1)\)-EXPTIME complete for disjunctive APT.

\subsection{Upper Bound}

We sketch a proof of the following theorem, based on Kobayashi and Ong's type system for recursion schemes~\cite{KO09LICS}.
An alternative proof, based on variable profiles~\cite{Ong06LICS}, is given in Appendix~\ref{app:alt-proof}.
\begin{theorem}\label{lem:pdisj}
 Let $\GRAM$ be an order-$n$ tree-generating recursion scheme and
 $\mathcal{B}$ a disjunctive APT. It can be decided in
 $(n-1)$-EXPTIME whether $\mathcal{B}$ accepts the value tree
 $\sem{\GRAM}$ from its root.
\end{theorem}

In a recent preprint \cite{KO09LICS},
%\lo{I think we should make the paper available on the web, and give a URL in the bib reference.}\nk{Done. In the reference, I replaced ``preprint'' with ``submitted,'' to explicitly signal that the related paper is simultaneously submitted elsewhere.} \lo{Good idea.}
we constructed
an intersection type system {equivalent to the modal mu-calculus model checking of
recursion schemes, in the sense that
the tree generated by a recursion scheme is accepted by an APT if, and only if,
the recursion scheme is well-typed (in our type system)}.
Thus, the model checking problem is reduced to a type checking problem.
The main idea of the type system is to refine the tree type \(\T\)
by using the states and priorities of an APT: The type \(q\) describes a tree that is accepted
by the APT with \(q\) as the start state.
The intersection type \((\theta_1,m_1)\land (\theta_2,m_2)\ra q\), which refines the type \(\T\ra \T\),
describes a tree function that takes
an argument which has types \(\theta_1\) and \(\theta_2\), and returns
a tree of type \(q\).

The type checking algorithm presented in \emph{ibid.}~is \(n\)-EXPTIME in the combined size of the order-$n$ recursion scheme
and APT (more precisely, \(n\)-EXPTIME in
the largest arity of symbols in the recursion scheme,
the number of states of the APT, and the largest priory,
but polynomial in the number of the rules of the recursion scheme).
The bottleneck of the algorithm is the number of (atomic) intersection types,
where the set \(\AtomTy{\kappa}\) of atomic types refining a simple type \(\kappa\)
is inductively defined by:
\iffull
\[
\begin{array}{l}
\AtomTy{\T} = Q \\
\AtomTy{\kappa_1\ra \kappa_2} = \set{\IT S \ra \EAT \mid \EAT\in \AtomTy{\kappa_2}, S\subseteq \AtomTy{\kappa_1}\times P}
\end{array}
\]
\else
\(\AtomTy{\T} = Q\) and
\(\AtomTy{\kappa_1\ra \kappa_2} = \set{\IT S \ra \EAT \mid \EAT\in \AtomTy{\kappa_2}, S\subseteq \AtomTy{\kappa_1}\times P}\),
\fi
where \(Q\) and \(P\) are the sets of states and priorities respectively.
%%%\EAT^{\kappa_1\ra \cdots \ra \kappa_k\ra \T}
%%%::= \IT_{i\in I_1}(\EAT_{1,i}^{\kappa_1}, m_{1,i})
%%%\ra \cdots \ra \IT_{i\in I_k}(\EAT_{k,i}^{\kappa_k}, m_{k,i})\ra q\]
%%%Intuitively, \(q\) describes a tree accepted when the APT is run from state \(q\).
%%%Furthermore, the tree function can use an argument as
%%%a value of type \(\theta_i\) only when the largest priority visited is exactly \(m_i\):
%%%See \cite{KO09LICS} for more explanation.

According to the syntax of atomic types above,
the number of atomic types refining a simple type of order-\(n\)
is \(n\)-exponential in general.
In the case of disjunctive APT, however, for each type
of the form \(\T\ra\cdots \ra \T\ra \T\), we need to consider
only atomic types of the form \(\IT S_1 \ra \cdots \ra \IT S_k \ra q\), where
at most one of the \(S_i\)'s is a singleton set and the other \(S_j\)'s are empty.
Intuitively, this is because a run-tree of a disjunctive APT consists of a single path, so that
the run-tree visits only one of the arguments, at most once.
%%%Thus,
%%%we need to capture by an atomic type of order-\(1\) only information about
%%%which argument is visited and in which state
In fact, we can show that,
 if a recursion scheme is typable in
the type system for a disjunctive APT, the recursion scheme is typable
in a {restricted type system in which order-\(1\) types are constrained as described above}: this follows from the proof of completeness of the type
system~\cite{KO09LICS}, along with the property of the accepting run-tree mentioned
above.
Thus, the number of atomic types is \(k\times |Q|\times \changed{|P|}\times |Q|\)
(whereas for general APT, it is exponential). Therefore,
the number of atomic types possibly assigned to a symbol of order \(n\) is
\((n-1)\)-exponental. By running the same type checking algorithm as \emph{ibid.}~(but with {order-\(1\) types constrained} as above),
order-$n$ recursion schemes can be type-checked (i.e.~model-checked) in \((n-1)\)-EXPTIME.


\subsection{Lower Bound}
\label{disjunctiveAPT:lower-bound}

We show the lower bound by a reduction of the emptiness problem of the finite-word
language accepted by an order-$n$ (deterministic) PDA (which is $(n-1)$-EXPTIME complete \cite{Engelfriet91}).
From an order-$n$ PDA \(\APDA\), we can construct an order-$n$ tree-generating PDA \(\tPDA_{\APDA}{}\),
which simulates all possible input and \(\epsilon\)-transitions of \(\APDA\), and outputs \(\terminal{e}\)
only when \(\APDA\) reaches a final state: See Appendix~\ref{app:disjunctiAPT:lower-bound}.
By a result of Knapik et al.~\cite{Knapik02FOSSACS}, we can construct an
equi-expressive order-$n$ safe recursion scheme \(\GRAM\).
By the construction, the finite word-language accepted by \(\APDA\) is non-empty if, and only if,
the value tree of \(\GRAM\) has {a node labelled \(\terminal{e}\)}. Since the latter property can be expressed
by a disjunctive APT, the problem of model-checking recursion schemes for disjunctive APT is
\((n-1)\)-EXPTIME hard.
%%%We show that the model checking problem is \((n-1)\)-EXPTIME hard, by
%%%a reduction of the emptiness problem of the finite-word language generated by
%%%an order-$n$ \lochanged{(non-deterministic)} PDA (which is $(n-1)$-EXPTIME complete \cite{Engelfriet91})
%%%to the acceptance problem of the tree generated by a recursion scheme by a disjunctive APT.
%%%\nk{Here, the PDA is non-deterministic, right? } \lo{Yes.}

%%%Let \(\PDA\) be an order-$n$ PDA for generating a finite-word language.
%%%By a result of Knapik et al.~\cite{Knapik02FOSSACS},
%%%we can construct \changed{an}
%%%equi-expressive order-$n$ \emph{non-deterministic} safe recursion scheme \(\GRAM\) that generates a word language.
%%%\nk{This is the only place where we use \emph{non-deterministic} recursion schemes and
%%%\emph{non-deterministic} word-generating PDA.
%%%Since Engelfriet's original result is about a word-accepting DPDA, how about encoding it into
%%%a \emph{deterministic} tree-generating PDA whose path languages is the same (except
%%%some auxiliary symbols to express branching, like $\terminal{br}$) as the language accepted by the DPDA
%%%(and then transforming it into a deterministic recursion scheme)?
%%%} \lo{This is fine.}
%%%Further, we can encode \(\GRAM\) into a \emph{deterministic} order-$n$ tree-generating recursion scheme \(\GRAM'\),
%%%by replacing each rule
%%%\[
%%%    F \, x_1 \cdots x_n \; \rightarrow t_1 \; | \; \cdots \; | \; t_m
%%%\]
%%%  with
%%%\[
%%%    F \, x_1 \cdots x_n \; \rightarrow \; h \; t_1 (h \; t_2 (\cdots (h \; t_{m-1} \; (d\;t_m))))
%%%\]
%%%and replacing each terminal \(c\) of arity \(0\) with \(c \, E\) \lochanged{where $E$ is a fresh non-terminal} (thus \(c\) has arity \(1\) now), with a new rule \(E \Hra e \, E\).
%%%The terminal \(h\) represents a non-deterministic branch in $\GRAM$, while \(e\) corresponds to an \emph{end-of-string} marker. The arity-1 terminal \(d\) is inserted to ensure that the value tree of \(\GRAM'\) does not contain \(\bot\). \lo{I think this needs some clarification.}
%%%
%%%By the construction above, the followings are equivalent:
%%%\begin{enumerate}
%%%\item The finite-word language generated by \(\APDA\) is \lochanged{non-empty}.
%%%\item The value tree of \(\GRAM'\) has an occurence of \(e\).
%%%\end{enumerate}
%%%The latter property can easily be expressed by a disjunctive APT.
%%%Thus, the problem of checking recursion schemes for disjunctive APT is
%%%\((n-1)\)-EXPTIME hard.

As we show in Appendix~\ref{sec:n-1EXPTIME-in-APT}, the problem is
\((n-1)\)-EXPTIME hard also in the size of the disjunctive APT.
%\nk{Should we give more words on this result?} \nk{I wonder if the rest of this section is really necessary. In the next section, the result shown above is sufficient. The proof of the lower-bound shows that the reachability is \(n\)-EXPTIME hard, and that is sufficient for the purpose of discussing the complexity of resource usage verification. At least in the short version, just a remark that, from the above result, it follows that the verification problem of path properties is also \((n-1)\)-EXPTIME complete.}

\nk{I have restored a summary of the result about path properties, as they are mentioned in Introduction and Conclusion.} \lo{I like your summary - it says all the important things.}
\nk{I have removed the longer version of the section also from the full version, as it does not seem to contain much more information than the summary below.} \lo{Fine.}

%%\iffull\else
\subsection{Path Properties}
\label{sec:path-properties}
\lochanged{The \emph{path language} of a $\Sigma$-labelled tree $t$ is the image of the map $F$, which acts on the elements of the branch language of $t$ by ``forgetting the argument positions'' i.e.~$F : (f_1, d_1) \, (f_2, d_2) \cdots \mapsto f_1 \, f_2 \cdots$ and $F : (f_1, d_1) \cdots (f_n, d_n) \, \changed{f_{n+1}} \mapsto f_1 \cdots f_n \, \changed{f_{n+1}}$.}
We write \(\pathlang(\GRAM)\) for the \emph{path language} of \(\GRAM\).
%\lo{We need to give a proper definition of path language, in any case. I will do that next.} \lo{Done.}
For example, the path language of the tree $f \, a \, (f \, a \, b)$ is
$\set{fa, ffa, ffb}$.
%%%$\set{fa^\omega, ffa^\omega, ffb^\omega}$.
Thus elements of $\pathlang(\GRAM)$ are (possibly infinite) words over the alphabet $\Sigma$ which is now considered unranked (i.e.~arities of the symbols are forgotten).

Let \(\WA\) be a \emph{non-deterministic} parity word automaton (essentially
a disjunctive APT where all the terminal symbols have arity \(0\) or \(1\)).
We write \(\lang(\WA)\) for the word language accepted by \(\WA\).
By the result above, the problem \(\pathlang(\GRAM)\cap \lang(\WA)\stackrel{?}{=}\emptyset\) is \((n-1)\)-EXPTIME complete.
The decision problems \lochanged{\textsc{Reachability}} (i.e.~whether \(\sem{\GRAM}\) has a node labelled by a given symbol \(\terminal{e}\))
and \lochanged{\textsc{Finiteness}} (i.e.~whether \(\sem{\GRAM}\) is finite) are instances of the problem; hence they
are in \((n-1)\)-EXPTIME (the former is \((n-1)\)-EXPTIME complete, by the proof of Section~\ref{disjunctiveAPT:lower-bound}).

\lo{I am not able to show that \textsc{Finiteness} is $(n-1)$-EXPTIME hard, but one can for a ``non-deterministic'' variant of the problem. We define the problem \textsc{ND-Infinity} as: given a non-deterministic recursion scheme $\GRAM$, does $\sem{\GRAM}$ contain an infinite tree? (equivalently, does the forest $\sem{\GRAM}$ have an infinite branch?) Let \({\cal A} \; := \; \langle P, p_0\in P, \Gamma, {\Sigma},
  \delta, F\subseteq P\rangle\) be an order-$n$ deterministic PDA where \(\delta\) is a partial function from
\(P\times \Gamma\times ({\Sigma}\cup\set{\epsilon})\) to \(P\times \OP{n}\). We define a \emph{non-deterministic} order-$n$ PDA (generating a language of $\set{\terminal{e}, \bot}$-ranked trees)
\[\tPDA_{\APDA}{} \; := \;
   \langle \set{\terminal{e}, \bot}, \; \Gamma, \;
   P, \; \delta' : P \times \Gamma \longrightarrow {\cal P}(P \times \OP{n} + \set{(\terminal{e}; p) : p \in P}), \; p_0 \in P \rangle\]
where:
\[\delta'(p, \gamma) \; :=
\;
\left\{
\begin{array}{ll}
\set{(\terminal{e}; p)} & \hbox{if $p \in F$}\\
\set{(p', \theta) : \exists \alpha \in \Sigma \cup \set{\epsilon} \, . \, \delta(p, \alpha, \gamma) = (p', \theta)} & \hbox{otherwise}\\
\end{array}
\right.
\]
The language generated by $\tPDA_{\cal A}$ consists of at most two trees, namely, $\terminal{e} \, \terminal{e} \cdots$ and $\bot$. The idea is that the word language ${\cal L}({\cal A})$ is non-empty if, and only if, the language generated by $\tPDA_{\cal A}$ contains the infinite tree $\terminal{e} \, \terminal{e} \cdots$. Thus, it follows from Engelfriet's result and the equi-expressivity result (for tree languages) of Knapik et al.~that \textsc{ND-Infinity} is $(n-1)$-EXPTIME hard.}


%%\fi



%%%\subsection{Applications: Complexity of Verification of Path Properties}
%%%
%%%\lochanged{Henceforth, without loss of generality, we assume that the tree generated by a recursion scheme does not have any finite branches.}
%%%\nk{Actually, in the finiteness problem, we do consider a recursion scheme producing finite branches.
%%%Is there any reason why we should not define \(\pathlang(\GRAM)\) as a subset of \(\Sigma^*\cup\Sigma^\omega\)?}
%%%
%%%\lo{The main reason is that results in the literature are, in the main, either for finite-word languages or for infinite-word languages, but not for a mixture. This seems clearly so in the automata-theoretic approach. The standard automata (B\"uchi, Muller, Parity, etc.) are defined to accept only infinite words. I think what we could do is to define the path language $\pathlang(\GRAM)$ to be a subset of $\Sigma^\ast \cup \Sigma^\omega$, and then define ${\cal W}^\omega(\GRAM)$ (say) to be a canonical embedding of $\pathlang(\GRAM)$ into ${\cal P}(\Sigma^\omega)$. What do you think? }
%%%We write \(\pathlang(\GRAM)\) for the \emph{path language} of \(\GRAM\), consisting of
%%%paths in the value tree \(\sem{\GRAM}\).
%%%\lo{We need to give a proper definition of path language, in any case. I will do that next.}
%%%For example, the path language of the tree $f \, a \, (f \, a \, b)$ is $\set{fa^\omega, ffa^\omega, ffb^\omega}$.
%%%Thus elements of $\pathlang(\GRAM)$ are infinite words over the alphabet $\Sigma$ which is now considered unranked (i.e.~arities of the symbols are forgotten).
%%%
%%%\lo{We sometimes write $\pathlang(\sem{\GRAM})$ for $\pathlang(\GRAM)$. For consistency, I have replaced all occurrences of the former by the latter.}
%%%
%%%\nk{Here, do you mean by $\omega$-words only infinite words, excluding finite words?
%%%In that case, we should probably say that any recursion scheme generating a value tree containing a finite branch can be transformed into a ``completely infinite'' tree, by replacing each terminal \(c\) of arity \(0\) with \(c E\), with a rule \(E\ra e(E)\).} \lo{Yes. Implemented.}
%%%
%%%
%%%\paragraph{The problem: $\pathlang(\GRAM) \cap \mathcal{L}(\WA) \; \stackrel{?}{=} \; \emptyset$}
%%%
%%%Let $\WA = \anglebra{Q, \, \Sigma, \, \Delta \subseteq Q \times \Sigma \times Q, \, \Omega : Q \longrightarrow \set{1, \cdots, p}}$ be
%%%a \emph{non-deterministic} parity word automaton,
%%%where the priority function $\Omega$ is not assumed to be
%%%trivial. (B\"uchi automata are equivalent to parity automata with two
%%%colours or priorities.)
%%%\nk{Should we give the definition of parity word automata? Too many automata appear in
%%%the paper, and probably we do not have enough space for explaining all of them; perhaps move the definitions of relatively well-known automata to appendices?} \lo{Yes. I think we should do that.} Writing $\mathcal{L}(\WA)$ for the language
%%%recognized by $\WA$, we have $\pathlang(\GRAM) \cap \mathcal{L}(\WA) \, \neq \, \emptyset$ if, and only if, $\sem{\GRAM}$ is accepted by the APT
%%%\[\mathcal{B} \; = \; \anglebra{Q, \, \Sigma, \, \delta : Q \times \Sigma
%%%\longrightarrow {\mathsf B}^+([\arity(\Sigma)]  \times Q), \, \Omega}\]
%%%with the following \emph{disjunctive} transition function
%%%\[\delta \; : \; (q, f) \; \mapsto \; %\bigvee_{1 \leq i \leq \arity(f)} \; \bigvee_{p \, : \, (q, f, p) \in \Delta}
%%%\bigvee \set{(i, p) : 1 \leq i \leq \arity(f), (q, f, p) \in \Delta}.\]
%%%
%%%It follows from Lemma~\ref{lem:pdisj} that the problem $\pathlang(\GRAM) \cap \mathcal{L}(\WA) \, \stackrel{?}{=} \, \emptyset$ can be decided in $(n-1)$-EXPTIME.
%%%
%%%Let \(\WA\) be a parity word automaton that accepts \lochanged{\(\Sigma^* e^\omega\)}, and \(\GRAM'\) be the recursion scheme
%%%in Section~\ref{disjunctiveAPT:lower-bound}.
%%%Then, \(\pathlang(\GRAM') \cap \mathcal{L}(\WA) \; \neq \; \emptyset\) if, and only if,
%%%\(\GRAM'\) has a \lochanged{node labelled \(e\)}. Thus, the problem
%%%$\pathlang(\GRAM) \cap \mathcal{L}(\WA) \; \stackrel{?}{=} \; \emptyset$
%%%is also  $(n-1)$-EXPTIME-hard.
%%%
%%%
%%%\paragraph{The problem: $\pathlang(\GRAM) \; \stackrel{?}{\subseteq} \; \mathcal{L}(\WA)$}
%%%
%%%Let $\WA$ be a \emph{deterministic} parity word automaton
%%%\[\WA \; = \; \anglebra{Q, \; \Sigma, \; \delta_{\WA} :
%%%Q \times \Sigma \longrightarrow Q,  \; q_0, \; \Omega : Q \longrightarrow \set{1, \cdots, p}}.\]
%%%Define $\overline A := \anglebra{Q, \Sigma,
%%%\delta_{\WA}, q_0, \overline \Omega}$ where $\overline \Omega : q \mapsto
%%%(\Omega(q) + 1)$. Note that because of determinacy,
%%%$\mathcal{L}(\overline {\WA}) = \Sigma^\omega \setminus \mathcal{L}(\WA)$. Now we have
%%%$\pathlang(\GRAM) \subseteq \lang(\WA)$ if, and only if,
%%%$\pathlang(\GRAM) \cap \lang(\overline{\WA}) =\emptyset$.
%%%Thus, the problem  $\pathlang(\GRAM) \; \stackrel{?}{\subseteq} \; \mathcal{L}(\WA)$
%%%is \((n-1)\)-EXPTIME. Moreover, since the language \(\Sigma^* e^\omega\) is accepted by
%%%a deterministic parity \lochanged{word} automaton, the problem is also \((n-1)\)-EXPTIME hard.
%%%
%%%\paragraph{Reachability}
%%%The reachability is the problem of deciding whether \lochanged{\(\pathlang(\GRAM)\)} contains a given symbol \(\Tc\).
%%%This is an instance of the problem
%%%$\pathlang(\GRAM) \cap \mathcal{L}(\WA) \; \stackrel{?}{=} \; \emptyset$,
%%%where \(\WA\) is an automaton that accepts \(\Sigma^* \Tc\Sigma^\omega\).
%%%Thus, the problem is \((n-1)\)-EXPTIME complete (the lower bound follows exactly the same argument as the proof in Section~\ref{disjunctiveAPT:lower-bound}).
%%%
%%%\paragraph{Finiteness}
%%%The finiteness is the problem of deciding whether all words in \(\pathlang(\GRAM)\) are infinite.
%%%This can be encoded into the problem
%%%$\pathlang(\GRAM')\; \stackrel{?}{\subseteq} \; \mathcal{L}(\WA)$,
%%%where \(\GRAM'\) is obtained by
%%%replacing each occurrence of arity-0 terminal \(\Tc\) with \(\Tc(E)\) and adding the rule \(E\Hra \Te(E)\),
%%%and \(\WA\) is an automaton that accepts \(\Sigma^* \Te^\omega\).
%%%Thus, the finiteness problem is \((n-1)\)-EXPTIME.
%%%We do not know whether the problem is \((n-1)\)-EXPTIME-hard.
%%%
%%%



==> path.tex <==
\section{Disjunctive APT and Complexity of Model Checking}
\label{sec:disjunctiveAPT}

%%\nk{I have restructured this section to make the structure similar to
%%that of the previous section: first introduce a subclass of APT, and
%%then analyze the complexity of the model checking problem.} \lo{This
%%is fine.}

\newcommand\pathlang[1]{\mathcal{W}\,{#1}}
\newcommand\vp{\hbox{\bf VP}}
\newcommand\cgraph[1]{\mathit{Gr}_{#1}}

%%\section{(\(n-1\))-EXPTIME-Completeness of Verification of Path Properties}

%\subsection{Disjunctive APT}

%\lo{It seems a little odd that, in contrast to trivial APT, the logical characterization of disjunctive APT is relegated to Appendix~\ref{sec:equi-expressivity}. For this reason, and following the pattern of the preceding section, I have (i) inserted a subsection (ii) introduced the ``disjunctive fragment'' (iii) changed the footnote to a remark. If you are not happy with any of the above, please feel free to change it back.}

A \emph{disjunctive APT} is an APT whose transition function
\(\delta\) is disjunctive, i.e.~the image of \(\delta\) consists of positive boolean formulas that contain only disjunctions and no conjunctions, as given by the grammar
\(\theta \; ::= \; \TRUE \; | \; \FALSE \; | \; (i, q) \; | \;  \theta \vee \theta \).
Disjunctive APT can be used to describe path (or linear-time) properties of trees.

%\lochanged{
First we give a logical characterization of disjunctive APT as follows. Call $\cal D$ the following ``disjunctive fragment'' of the modal mu-calculus:
\[\phi, \psi \; ::= \; P_f \wedge \phi
%\; | \; (\neg P_f) \wedge \phi
\; | \; Z
\; | \; \phi \vee \psi
\; | \; \diaform{i}{\phi}
\; | \; \nuform{Z}{\phi}
\; | \; \muform{Z}{\phi}
\]
where $f$ ranges over symbols in $\Sigma$, and $i$ ranges over $\set{1, \cdots, \arity(\Sigma)}$.
A proof is given in Appendix~\ref{sec:equi-expressivity}.
%}

\begin{proposition}[Equi-Expressivity]
\label{prop:equi-expressivity2}
The logic $\cal D$ and %%B\"uchi automata
disjunctive APT are equivalent for defining possibly-infinite
ranked trees. I.e.~for every closed $\cal D$-formula, there is a disjunctive APT that defines the same tree language, and vice versa.
\end{proposition}

\begin{remark}\rm \begin{inparaenum}[(i)]
\item Note that a disjunctive APT is a non-deterministic parity tree automaton.
\item For defining languages of ranked trees, disjunctive APT (or rather the formulas corresponding to them) are a proper subset of the \emph{disjunctive formulas} in the sense of Walukiewicz and Janin  \cite{JW95}. (Satisfiability checking of these disjunctive formulas is linear time.) For example, the disjunctive formula $(1 \rightarrow \set{{\sf t}}) \wedge (2 \rightarrow \set{{\sf t}})$ is not equivalent to any disjunctive APT.
\end{inparaenum}
\end{remark}
%}
%\nk{I have moved the remark here, due to the lack of space.}
%%\lo{ICALP referees who are aware of Walukiewicz' notion of \emph{disjunctive formulas} would likely query its connexion with disjunctive APT, hence the remark. We could also insert it as a footnote.}
%%\end{remark}
%%%It follows from the definition of (disjunctive) APT that, in case
%%%$\arity(a) = 0$, it is possible for $\delta(q, a) \in {\sf
%%%B}^+(\emptyset)$ to be $\sf t$ or $\sf f$.}} \nk{Make it clear whether
%%%we allow \(\TRUE\) when the arity is \(0\).}\lo{Done.}
%%\nk{Actually, it seems that we can allow \(\TRUE\) even in the case \(\arity(a)\neq 0\). Am I right?} \lo{Yes.}
%%%We then use the result to analyze the complexity of
%%%decision problems on the \lochanged{\emph{path languages} (of trees)} generated by recursion schemes. See Appendix~\ref{sec:equi-expressivity} for a logical characterization of disjunctive APT.

In the rest of the section, we show that the model checking problem for order-\(n\) recursion schemes is \((n-1)\)-EXPTIME complete for disjunctive APT.

\subsection{Upper Bound}

We sketch a proof of the following theorem, based on Kobayashi and Ong's type system for recursion schemes~\cite{KO09LICS}.
An alternative proof, based on variable profiles~\cite{Ong06LICS}, is given in Appendix~\ref{app:alt-proof}.
\begin{theorem}\label{lem:pdisj}
 Let $\GRAM$ be an order-$n$ tree-generating recursion scheme and
 $\mathcal{B}$ a disjunctive APT. It can be decided in
 $(n-1)$-EXPTIME whether $\mathcal{B}$ accepts the value tree
 $\sem{\GRAM}$ from its root.
\end{theorem}

In a recent preprint \cite{KO09LICS},
%\lo{I think we should make the paper available on the web, and give a URL in the bib reference.}\nk{Done. In the reference, I replaced ``preprint'' with ``submitted,'' to explicitly signal that the related paper is simultaneously submitted elsewhere.} \lo{Good idea.}
we constructed
an intersection type system {equivalent to the modal mu-calculus model checking of
recursion schemes, in the sense that
the tree generated by a recursion scheme is accepted by an APT if, and only if,
the recursion scheme is well-typed (in our type system)}.
Thus, the model checking problem is reduced to a type checking problem.
The main idea of the type system is to refine the tree type \(\T\)
by using the states and priorities of an APT: The type \(q\) describes a tree that is accepted
by the APT with \(q\) as the start state.
The intersection type \((\theta_1,m_1)\land (\theta_2,m_2)\ra q\), which refines the type \(\T\ra \T\),
describes a tree function that takes
an argument which has types \(\theta_1\) and \(\theta_2\), and returns
a tree of type \(q\).

The type checking algorithm presented in \emph{ibid.}~is \(n\)-EXPTIME in the combined size of the order-$n$ recursion scheme
and APT (more precisely, \(n\)-EXPTIME in
the largest arity of symbols in the recursion scheme,
the number of states of the APT, and the largest priory,
but polynomial in the number of the rules of the recursion scheme).
The bottleneck of the algorithm is the number of (atomic) intersection types,
where the set \(\AtomTy{\kappa}\) of atomic types refining a simple type \(\kappa\)
is inductively defined by:
\iffull
\[
\begin{array}{l}
\AtomTy{\T} = Q \\
\AtomTy{\kappa_1\ra \kappa_2} = \set{\IT S \ra \EAT \mid \EAT\in \AtomTy{\kappa_2}, S\subseteq \AtomTy{\kappa_1}\times P}
\end{array}
\]
\else
\(\AtomTy{\T} = Q\) and
\(\AtomTy{\kappa_1\ra \kappa_2} = \set{\IT S \ra \EAT \mid \EAT\in \AtomTy{\kappa_2}, S\subseteq \AtomTy{\kappa_1}\times P}\),
\fi
where \(Q\) and \(P\) are the sets of states and priorities respectively.
%%%\EAT^{\kappa_1\ra \cdots \ra \kappa_k\ra \T}
%%%::= \IT_{i\in I_1}(\EAT_{1,i}^{\kappa_1}, m_{1,i})
%%%\ra \cdots \ra \IT_{i\in I_k}(\EAT_{k,i}^{\kappa_k}, m_{k,i})\ra q\]
%%%Intuitively, \(q\) describes a tree accepted when the APT is run from state \(q\).
%%%Furthermore, the tree function can use an argument as
%%%a value of type \(\theta_i\) only when the largest priority visited is exactly \(m_i\):
%%%See \cite{KO09LICS} for more explanation.

According to the syntax of atomic types above,
the number of atomic types refining a simple type of order-\(n\)
is \(n\)-exponential in general.
In the case of disjunctive APT, however, for each type
of the form \(\T\ra\cdots \ra \T\ra \T\), we need to consider
only atomic types of the form \(\IT S_1 \ra \cdots \ra \IT S_k \ra q\), where
at most one of the \(S_i\)'s is a singleton set and the other \(S_j\)'s are empty.
Intuitively, this is because a run-tree of a disjunctive APT consists of a single path, so that
the run-tree visits only one of the arguments, at most once.
%%%Thus,
%%%we need to capture by an atomic type of order-\(1\) only information about
%%%which argument is visited and in which state
In fact, we can show that,
 if a recursion scheme is typable in
the type system for a disjunctive APT, the recursion scheme is typable
in a {restricted type system in which order-\(1\) types are constrained as described above}: this follows from the proof of completeness of the type
system~\cite{KO09LICS}, along with the property of the accepting run-tree mentioned
above.
Thus, the number of atomic types is \(k\times |Q|\times \changed{|P|}\times |Q|\)
(whereas for general APT, it is exponential). Therefore,
the number of atomic types possibly assigned to a symbol of order \(n\) is
\((n-1)\)-exponental. By running the same type checking algorithm as \emph{ibid.}~(but with {order-\(1\) types constrained} as above),
order-$n$ recursion schemes can be type-checked (i.e.~model-checked) in \((n-1)\)-EXPTIME.


\subsection{Lower Bound}
\label{disjunctiveAPT:lower-bound}

We show the lower bound by a reduction of the emptiness problem of the finite-word
language accepted by an order-$n$ (deterministic) PDA (which is $(n-1)$-EXPTIME complete \cite{Engelfriet91}).
From an order-$n$ PDA \(\APDA\), we can construct an order-$n$ tree-generating PDA \(\tPDA_{\APDA}{}\),
which simulates all possible input and \(\epsilon\)-transitions of \(\APDA\), and outputs \(\terminal{e}\)
only when \(\APDA\) reaches a final state: See Appendix~\ref{app:disjunctiAPT:lower-bound}.
By a result of Knapik et al.~\cite{Knapik02FOSSACS}, we can construct an
equi-expressive order-$n$ safe recursion scheme \(\GRAM\).
By the construction, the finite word-language accepted by \(\APDA\) is non-empty if, and only if,
the value tree of \(\GRAM\) has {a node labelled \(\terminal{e}\)}. Since the latter property can be expressed
by a disjunctive APT, the problem of model-checking recursion schemes for disjunctive APT is
\((n-1)\)-EXPTIME hard.
%%%We show that the model checking problem is \((n-1)\)-EXPTIME hard, by
%%%a reduction of the emptiness problem of the finite-word language generated by
%%%an order-$n$ \lochanged{(non-deterministic)} PDA (which is $(n-1)$-EXPTIME complete \cite{Engelfriet91})
%%%to the acceptance problem of the tree generated by a recursion scheme by a disjunctive APT.
%%%\nk{Here, the PDA is non-deterministic, right? } \lo{Yes.}

%%%Let \(\PDA\) be an order-$n$ PDA for generating a finite-word language.
%%%By a result of Knapik et al.~\cite{Knapik02FOSSACS},
%%%we can construct \changed{an}
%%%equi-expressive order-$n$ \emph{non-deterministic} safe recursion scheme \(\GRAM\) that generates a word language.
%%%\nk{This is the only place where we use \emph{non-deterministic} recursion schemes and
%%%\emph{non-deterministic} word-generating PDA.
%%%Since Engelfriet's original result is about a word-accepting DPDA, how about encoding it into
%%%a \emph{deterministic} tree-generating PDA whose path languages is the same (except
%%%some auxiliary symbols to express branching, like $\terminal{br}$) as the language accepted by the DPDA
%%%(and then transforming it into a deterministic recursion scheme)?
%%%} \lo{This is fine.}
%%%Further, we can encode \(\GRAM\) into a \emph{deterministic} order-$n$ tree-generating recursion scheme \(\GRAM'\),
%%%by replacing each rule
%%%\[
%%%    F \, x_1 \cdots x_n \; \rightarrow t_1 \; | \; \cdots \; | \; t_m
%%%\]
%%%  with
%%%\[
%%%    F \, x_1 \cdots x_n \; \rightarrow \; h \; t_1 (h \; t_2 (\cdots (h \; t_{m-1} \; (d\;t_m))))
%%%\]
%%%and replacing each terminal \(c\) of arity \(0\) with \(c \, E\) \lochanged{where $E$ is a fresh non-terminal} (thus \(c\) has arity \(1\) now), with a new rule \(E \Hra e \, E\).
%%%The terminal \(h\) represents a non-deterministic branch in $\GRAM$, while \(e\) corresponds to an \emph{end-of-string} marker. The arity-1 terminal \(d\) is inserted to ensure that the value tree of \(\GRAM'\) does not contain \(\bot\). \lo{I think this needs some clarification.}
%%%
%%%By the construction above, the followings are equivalent:
%%%\begin{enumerate}
%%%\item The finite-word language generated by \(\APDA\) is \lochanged{non-empty}.
%%%\item The value tree of \(\GRAM'\) has an occurence of \(e\).
%%%\end{enumerate}
%%%The latter property can easily be expressed by a disjunctive APT.
%%%Thus, the problem of checking recursion schemes for disjunctive APT is
%%%\((n-1)\)-EXPTIME hard.

As we show in Appendix~\ref{sec:n-1EXPTIME-in-APT}, the problem is
\((n-1)\)-EXPTIME hard also in the size of the disjunctive APT.
%\nk{Should we give more words on this result?} \nk{I wonder if the rest of this section is really necessary. In the next section, the result shown above is sufficient. The proof of the lower-bound shows that the reachability is \(n\)-EXPTIME hard, and that is sufficient for the purpose of discussing the complexity of resource usage verification. At least in the short version, just a remark that, from the above result, it follows that the verification problem of path properties is also \((n-1)\)-EXPTIME complete.}

%\nk{I have restored a summary of the result about path properties, as they are mentioned in Introduction and Conclusion.} \lo{I like your summary - it says all the important things.}
%\nk{I have removed the longer version of the section also from the full version, as it does not seem to contain much more information than the summary below.} \lo{Fine.}

%%\iffull\else
\subsection{Path Properties}
\label{sec:path-properties}
The \emph{path language} of a $\Sigma$-labelled tree $t$ is the image of the map $F$, which acts on the elements of the branch language of $t$ by ``forgetting the argument positions'' i.e.~$F : (f_1, d_1) \, (f_2, d_2) \cdots \mapsto f_1 \, f_2 \cdots$ and $F : (f_1, d_1) \cdots (f_n, d_n) \, \changed{f_{n+1}} \mapsto f_1 \cdots f_n \, \lochanged{f_{n+1}^\omega}$.
We write \(\pathlang(\GRAM)\) for the \emph{path language} of \(\GRAM\).
%\lo{We need to give a proper definition of path language, in any case. I will do that next.} \lo{Done.}
For example, the path language of the tree $f \, a \, (f \, a \, b)$ is
\lochanged{$\set{f\,a^\omega, f\,f\,a^\omega, f\,f\,b^\omega}$}.
%%%$\set{fa^\omega, ffa^\omega, ffb^\omega}$.
Thus elements of $\pathlang(\GRAM)$ are \lochanged{infinite} words over the alphabet $\Sigma$ which is now considered unranked (i.e.~arities of the symbols are forgotten).

Let \(\WA\) be a \emph{non-deterministic} parity word automaton (essentially
a disjunctive APT where all the terminal symbols have arity \(0\) or \(1\)).
We write \(\lang(\WA)\) for the word language accepted by \(\WA\).
By the result above, the problem \(\pathlang(\GRAM)\cap \lang(\WA)\stackrel{?}{=}\emptyset\) is \((n-1)\)-EXPTIME complete.
The decision problems \textsc{Reachability} (i.e.~whether \(\sem{\GRAM}\) has a node labelled by a given symbol \(\terminal{e}\))
and \textsc{Finiteness} (i.e.~whether \(\sem{\GRAM}\) is finite) are instances of the problem; hence they
are in \((n-1)\)-EXPTIME (the former is \((n-1)\)-EXPTIME complete, by the proof of Section~\ref{disjunctiveAPT:lower-bound}).

%\lo{I am not able to show that \textsc{Finiteness} is $(n-1)$-EXPTIME hard, but one can for a ``non-deterministic'' variant of the problem. We define the problem \textsc{ND-Infinity} as: given a non-deterministic recursion scheme $\GRAM$, does $\sem{\GRAM}$ contain an infinite tree? (equivalently, does the forest $\sem{\GRAM}$ have an infinite branch?) Let \({\cal A} \; := \; \langle P, p_0\in P, \Gamma, {\Sigma},
%  \delta, F\subseteq P\rangle\) be an order-$n$ deterministic PDA where \(\delta\) is a partial function from
%\(P\times \Gamma\times ({\Sigma}\cup\set{\epsilon})\) to \(P\times \OP{n}\). We define a \emph{non-deterministic} order-$n$ PDA (generating a language of $\set{\terminal{e}, \bot}$-ranked trees)
%\[\tPDA_{\APDA}{} \; := \;
%   \langle \set{\terminal{e}, \bot}, \; \Gamma, \;
%   P, \; \delta' : P \times \Gamma \longrightarrow {\cal P}(P \times \OP{n} + \set{(\terminal{e}; p) : p \in P}), \; p_0 \in P \rangle\]
%where:
%\[\delta'(p, \gamma) \; :=
%\;
%\left\{
%\begin{array}{ll}
%\set{(\terminal{e}; p)} & \hbox{if $p \in F$}\\
%\set{(p', \theta) : \exists \alpha \in \Sigma \cup \set{\epsilon} \, . \, \delta(p, \alpha, \gamma) = (p', \theta)} & \hbox{otherwise}\\
%\end{array}
%\right.
%\]
%The language generated by $\tPDA_{\cal A}$ consists of at most two trees, namely, $\terminal{e} \, \terminal{e} \cdots$ and $\bot$. The idea is that the word language ${\cal L}({\cal A})$ is non-empty if, and only if, the language generated by $\tPDA_{\cal A}$ contains the infinite tree $\terminal{e} \, \terminal{e} \cdots$. Thus, it follows from Engelfriet's result and the equi-expressivity result (for tree languages) of Knapik et al.~that \textsc{ND-Infinity} is $(n-1)$-EXPTIME hard.}


%%\fi



%%%\subsection{Applications: Complexity of Verification of Path Properties}
%%%
%%%\lochanged{Henceforth, without loss of generality, we assume that the tree generated by a recursion scheme does not have any finite branches.}
%%%\nk{Actually, in the finiteness problem, we do consider a recursion scheme producing finite branches.
%%%Is there any reason why we should not define \(\pathlang(\GRAM)\) as a subset of \(\Sigma^*\cup\Sigma^\omega\)?}
%%%
%%%\lo{The main reason is that results in the literature are, in the main, either for finite-word languages or for infinite-word languages, but not for a mixture. This seems clearly so in the automata-theoretic approach. The standard automata (B\"uchi, Muller, Parity, etc.) are defined to accept only infinite words. I think what we could do is to define the path language $\pathlang(\GRAM)$ to be a subset of $\Sigma^\ast \cup \Sigma^\omega$, and then define ${\cal W}^\omega(\GRAM)$ (say) to be a canonical embedding of $\pathlang(\GRAM)$ into ${\cal P}(\Sigma^\omega)$. What do you think? }
%%%We write \(\pathlang(\GRAM)\) for the \emph{path language} of \(\GRAM\), consisting of
%%%paths in the value tree \(\sem{\GRAM}\).
%%%\lo{We need to give a proper definition of path language, in any case. I will do that next.}
%%%For example, the path language of the tree $f \, a \, (f \, a \, b)$ is $\set{fa^\omega, ffa^\omega, ffb^\omega}$.
%%%Thus elements of $\pathlang(\GRAM)$ are infinite words over the alphabet $\Sigma$ which is now considered unranked (i.e.~arities of the symbols are forgotten).
%%%
%%%\lo{We sometimes write $\pathlang(\sem{\GRAM})$ for $\pathlang(\GRAM)$. For consistency, I have replaced all occurrences of the former by the latter.}
%%%
%%%\nk{Here, do you mean by $\omega$-words only infinite words, excluding finite words?
%%%In that case, we should probably say that any recursion scheme generating a value tree containing a finite branch can be transformed into a ``completely infinite'' tree, by replacing each terminal \(c\) of arity \(0\) with \(c E\), with a rule \(E\ra e(E)\).} \lo{Yes. Implemented.}
%%%
%%%
%%%\paragraph{The problem: $\pathlang(\GRAM) \cap \mathcal{L}(\WA) \; \stackrel{?}{=} \; \emptyset$}
%%%
%%%Let $\WA = \anglebra{Q, \, \Sigma, \, \Delta \subseteq Q \times \Sigma \times Q, \, \Omega : Q \longrightarrow \set{1, \cdots, p}}$ be
%%%a \emph{non-deterministic} parity word automaton,
%%%where the priority function $\Omega$ is not assumed to be
%%%trivial. (B\"uchi automata are equivalent to parity automata with two
%%%colours or priorities.)
%%%\nk{Should we give the definition of parity word automata? Too many automata appear in
%%%the paper, and probably we do not have enough space for explaining all of them; perhaps move the definitions of relatively well-known automata to appendices?} \lo{Yes. I think we should do that.} Writing $\mathcal{L}(\WA)$ for the language
%%%recognized by $\WA$, we have $\pathlang(\GRAM) \cap \mathcal{L}(\WA) \, \neq \, \emptyset$ if, and only if, $\sem{\GRAM}$ is accepted by the APT
%%%\[\mathcal{B} \; = \; \anglebra{Q, \, \Sigma, \, \delta : Q \times \Sigma
%%%\longrightarrow {\mathsf B}^+([\arity(\Sigma)]  \times Q), \, \Omega}\]
%%%with the following \emph{disjunctive} transition function
%%%\[\delta \; : \; (q, f) \; \mapsto \; %\bigvee_{1 \leq i \leq \arity(f)} \; \bigvee_{p \, : \, (q, f, p) \in \Delta}
%%%\bigvee \set{(i, p) : 1 \leq i \leq \arity(f), (q, f, p) \in \Delta}.\]
%%%
%%%It follows from Lemma~\ref{lem:pdisj} that the problem $\pathlang(\GRAM) \cap \mathcal{L}(\WA) \, \stackrel{?}{=} \, \emptyset$ can be decided in $(n-1)$-EXPTIME.
%%%
%%%Let \(\WA\) be a parity word automaton that accepts \lochanged{\(\Sigma^* e^\omega\)}, and \(\GRAM'\) be the recursion scheme
%%%in Section~\ref{disjunctiveAPT:lower-bound}.
%%%Then, \(\pathlang(\GRAM') \cap \mathcal{L}(\WA) \; \neq \; \emptyset\) if, and only if,
%%%\(\GRAM'\) has a \lochanged{node labelled \(e\)}. Thus, the problem
%%%$\pathlang(\GRAM) \cap \mathcal{L}(\WA) \; \stackrel{?}{=} \; \emptyset$
%%%is also  $(n-1)$-EXPTIME-hard.
%%%
%%%
%%%\paragraph{The problem: $\pathlang(\GRAM) \; \stackrel{?}{\subseteq} \; \mathcal{L}(\WA)$}
%%%
%%%Let $\WA$ be a \emph{deterministic} parity word automaton
%%%\[\WA \; = \; \anglebra{Q, \; \Sigma, \; \delta_{\WA} :
%%%Q \times \Sigma \longrightarrow Q,  \; q_0, \; \Omega : Q \longrightarrow \set{1, \cdots, p}}.\]
%%%Define $\overline A := \anglebra{Q, \Sigma,
%%%\delta_{\WA}, q_0, \overline \Omega}$ where $\overline \Omega : q \mapsto
%%%(\Omega(q) + 1)$. Note that because of determinacy,
%%%$\mathcal{L}(\overline {\WA}) = \Sigma^\omega \setminus \mathcal{L}(\WA)$. Now we have
%%%$\pathlang(\GRAM) \subseteq \lang(\WA)$ if, and only if,
%%%$\pathlang(\GRAM) \cap \lang(\overline{\WA}) =\emptyset$.
%%%Thus, the problem  $\pathlang(\GRAM) \; \stackrel{?}{\subseteq} \; \mathcal{L}(\WA)$
%%%is \((n-1)\)-EXPTIME. Moreover, since the language \(\Sigma^* e^\omega\) is accepted by
%%%a deterministic parity \lochanged{word} automaton, the problem is also \((n-1)\)-EXPTIME hard.
%%%
%%%\paragraph{Reachability}
%%%The reachability is the problem of deciding whether \lochanged{\(\pathlang(\GRAM)\)} contains a given symbol \(\Tc\).
%%%This is an instance of the problem
%%%$\pathlang(\GRAM) \cap \mathcal{L}(\WA) \; \stackrel{?}{=} \; \emptyset$,
%%%where \(\WA\) is an automaton that accepts \(\Sigma^* \Tc\Sigma^\omega\).
%%%Thus, the problem is \((n-1)\)-EXPTIME complete (the lower bound follows exactly the same argument as the proof in Section~\ref{disjunctiveAPT:lower-bound}).
%%%
%%%\paragraph{Finiteness}
%%%The finiteness is the problem of deciding whether all words in \(\pathlang(\GRAM)\) are infinite.
%%%This can be encoded into the problem
%%%$\pathlang(\GRAM')\; \stackrel{?}{\subseteq} \; \mathcal{L}(\WA)$,
%%%where \(\GRAM'\) is obtained by
%%%replacing each occurrence of arity-0 terminal \(\Tc\) with \(\Tc(E)\) and adding the rule \(E\Hra \Te(E)\),
%%%and \(\WA\) is an automaton that accepts \(\Sigma^* \Te^\omega\).
%%%Thus, the finiteness problem is \((n-1)\)-EXPTIME.
%%%We do not know whether the problem is \((n-1)\)-EXPTIME-hard.
%%%
%%%


